Adversarial Sets for Regularising Neural Link Predictors

In adversarial training, a set of models learn together by pursuing competing goals, usually defined on single data instances. However, in relational learning and other non-i.i.d domains, goals can also be defined over sets of instances. For example, a link predictor for the is-a relation needs to be consistent with the transitivity property: if is-a(x_1, x_2) and is-a(x_2, x_3) hold, is-a(x_1, x_3) needs to hold as well. Here we use such assumptions for deriving an inconsistency loss, measuring the degree to which the model violates the assumptions on an adversarially-generated set of examples. The training objective is defined as a minimax problem, where an adversary finds the most offending adversarial examples by maximising the inconsistency loss, and the model is trained by jointly minimising a supervised loss and the inconsistency loss on the adversarial examples. This yields the first method that can use function-free Horn clauses (as in Datalog) to regularise any neural link predictor, with complexity independent of the domain size. We show that for several link prediction models, the optimisation problem faced by the adversary has efficient closed-form solutions. Experiments on link prediction benchmarks indicate that given suitable prior knowledge, our method can significantly improve neural link predictors on all relevant metrics.

==> adversarial.tex <==
% !TeX spellcheck = en_GB

\section{Adversarial Rule Injection} \label{sec:injection}

%
In this section we propose \emph{Adversarial Rule Injection} (\ARI), an efficient method for incorporating first-order rules in Knowledge Graph embedding models.
%

%
An \emph{atom} is a fact (triple) that can have variables at the subject and/or object position.
%
A \emph{First-Order rule} consists of an implication between a \emph{body} and an \emph{head}, where the head is a single atom, and the body is a set of atoms.
%
Let $\vars$ be a set of universally quantified %set of
variables.
%
We denote a rule with head $\relq(x_{1}, x_{2})$ and body $\{ B_{1}, \ldots, B_{n} \}$ by an implication:
%
\begin{equation} \label{eq:rule}
%
 B_{1} \land B_{2} \land \ldots \land B_{m} \Implies \relq(x_{1}, x_{2})
%
\end{equation}
%
\noindent where each $x_{1}, x_{2} \in \vars$ are two variables in $\vars$, $\relq \in \rels$, and each $B_{i}$ is an atom $\rp(x_{i, 1}, x_{i, 2})$ with $\rp \in \rels$ and $x_{i, 1}, x_{i, 2} \in \vars$.
%
We abbreviate the rule in Eq.~\ref{eq:rule} by $\vec{B} \Implies \relq(x_{1}, x_{2})$.

%
An \emph{instantiation} of a rule is a copy of the rule where all variables in $\vars$ have been substituted by entities in $\ents$.
%
According to the rule in Eq.~\ref{eq:rule} is that for any instantiation of the rule, if the body holds, then the head also holds.
%

%
\thms{why sibling (which can be female)? replace sibling by brother?}
\begin{example}
%
Consider the sentence ``\emph{An uncle is a sibling of a parent}''.
%
It can be encoded by the following rule:
%
\begin{equation} \label{eq:rulex}
 \rel{siblingOf}(x_{1}, x_{2}) \land \rel{parentOf}(x_{2}, x_{3}) \Implies \rel{uncleOf}(x_{1}, x_{3}),
\end{equation}
%
\noindent where $\vars = \{ x_{1}, x_{2}, x_{3} \}$ is the set of variables, $\rel{uncleOf}(x_{1}, x_{3})$ is the head and $\rel{siblingOf}(x_{1}, x_{2}) \land \rel{parentOf}(x_{2}, x_{3})$ the body of the rule.
%

%
Assume $\{ \ent{Mark}, \ent{John}, \ent{Paul} \} \subseteq \ents$: according to the rule in Eq.~\ref{eq:rulex}, if $\rel{siblingOf}(\ent{Mark}, \ent{John})$ and $\rel{parentOf}(\ent{John}, \ent{Paul})$ hold, then $\rel{uncleOf}(\ent{Mark}, \ent{Paul})$ also holds.
%
\end{example}
%

%
\subsection{Grounded Loss Formulation}
%

Following \cite{DBLP:conf/emnlp/DemeesterRR16}, an implication rule in the form:
%
\begin{equation} \label{eq:simple}
%
 \rp(x_{1}, x_{2}) \Implies \relq(x_{1}, x_{2}),
%
\end{equation}
%
\noindent with $\vars = \{ x_{1}, x_{2} \}$, can be enforced by requiring that, for every pair of entities $\pair{\rs}{\ro} \in \ents \times \ents$, the triple $\spo$ is considered less likely than the triple $\sqo$, \ie:
%
\begin{equation} \label{eq:csimple}
%
 \forall \rs, \ro \in \ents : \fscore(\spo) \leq \fscore(\sqo).
%
\end{equation}
%
Note that if $\spo$ is a true fact with a high score $\fscore(\spo)$, and the fact $\sqo$ has an higher score, it must also be true, but not vice-versa.
%
We can thus enforce an implication rule by minimizing a loss term with a separate contribution for every $\pair{\rs}{\ro} \in \ents \times \ents$, adding up to the loss function in Eq.~\ref{eq:loss} if the corresponding inequality is not satisfied.
%
The implication loss for the rule in Eq.~\ref{eq:simple} can be formulated as:
%
\begin{equation} \label{eq:lsimple}
%
 \loss_{G}(\params) = \sum_{\rs \in \ents} \sum_{\ro \in \ents} \hinge{\fscore(\spo ; \params) - \fscore(\sqo ; \params)}.
%
\end{equation}
%
Note that the loss function $\loss_{G}(\params)$ in Eq.~\ref{eq:lsimple} reaches its global minimum $0$ when parameters $\params$ match the constraints in Eq.~\ref{eq:csimple}, and it is strictly positive otherwise.
%

%
However, a limitation of implication rules in the form provided in Eq.~\ref{eq:simple} is that the body is limited to one single atom.
%
Following \cite{DBLP:conf/naacl/RocktaschelSR15}, the score for a conjunction of atoms can be computed using \emph{t-norms}~\cite{Gupta:1991:TTN:107687.107690}, for instance:
%
\begin{itemize}
%
 \item The \emph{Minimum t-norm}, also called \emph{Zadeh's t-norm}:
 \[ \fscore(\langle \rs_{1}, \rp_{1}, \ro_{1} \rangle \land \langle \rs_{2}, \rp_{2}, \ro_{2} \rangle) = \min \left\{ \fscore(\langle \rs_{1}, \rp_{1}, \ro_{1} \rangle), \fscore(\langle \rs_{2}, \rp_{2}, \ro_{2} \rangle) \right\} \]
%
 \item The \emph{Product t-norm}:
 \[ \fscore(\langle \rs_{1}, \rp_{1}, \ro_{1} \rangle \land \langle \rs_{2}, \rp_{2}, \ro_{2} \rangle) = \fscore(\langle \rs_{1}, \rp_{1}, \ro_{1} \rangle) \cdot \fscore(\langle \rs_{2}, \rp_{2}, \ro_{2} \rangle) \]
%
\end{itemize}
%

%
Let $\vars = \{ x_{1}, \ldots, x_{n} \}$, and let $x_{i} \equiv e$ denote the assignment of entity $e \in \ents$ to variable $x_{i} \in \vars$.
%
Given an implication rule in the form provided in Eq.~\ref{eq:rule}, its loss can be computed as follows:
%
\begin{equation} \label{eq:lrule}
%
 \loss_{G}(\params) = \sum_{\substack{e_{1} \in \ents \\ x_{1} \equiv e_{1}}} \ldots \sum_{\substack{e_{n} \in \ents \\ x_{n} \equiv e_{n}}} \hinge{\fscore(\vec{B} ; \params) - \fscore(\trpl{x_{1}}{\relq}{x_{2}} ; \params)}
%
\end{equation}
%

However, note that the loss in Eq.~\ref{eq:lrule} requires adding $\BigO{\card{\ents}^{n}}$ independent terms to the loss function.
%
Even for a small value of $n$, this can be unfeasible for real world Knowledge Graphs, which may contains millions of entities or more.
%

%
\subsection{Lifted Adversarial Loss Formulation}
%

%
\begin{algorithm}[t]
	\caption{Solving the minimax problem in Eq.~\ref{eq:minimax} via Stochastic Gradient Descent} \label{alg:sgd}
	\begin{algorithmic}[1]
		\REQUIRE{No. of training epochs $\tau_{a}, \tau_{d}, \tau$}
		\STATE{Randomly initialise model parameters $\params_{0}$}
		\FOR{$i \in \langle 1, \ldots, \tau \rangle$}
		\STATE{$\Aemb_{i} \leftarrow \textsc{FindAversarialExamples}(\params_{i - 1}, \tau_{a})$}
		\STATE{$\params_{i} \leftarrow \textsc{TrainModelParameters}(\Aemb_{i}, \tau_{d})$}
		\ENDFOR
		\STATE{\textbf{return} $\Theta_{\tau}$}
	\end{algorithmic}
	
	\begin{algorithmic}[1]
		\STATE{\textbf{function}\ \texttt{FindAdversarialExamples}($\params, \tau_{a}$)}
		\STATE{\{Solve the loss maximization problem in Eq.~\ref{eq:oadversary}\}}
		\STATE{Randomly initialise $\Aemb_{0}$}
		\FOR{$i \in \langle 1, \ldots, \tau_{a} \rangle$}
		\STATE{$\emb{} \leftarrow \emb{} / \norm{\emb{}}, \; \forall \emb{} \in \Aemb$}
		\STATE{$g_{i} \leftarrow  \nabla_{\Aemb} \loss_{A}(\Aemb)$}
		\STATE{$\Aemb_{i} \leftarrow \Aemb_{i - 1} + \eta_{i} g_{i}$}
		\ENDFOR
		\STATE{\textbf{return} $\Aemb_{\tau}$}
	\end{algorithmic}
	
	\begin{algorithmic}[1]
		\STATE{\textbf{function}\ \texttt{TrainModelParameters}($\Aemb, \tau_{d})$}
		\STATE{\{Solve the loss minimization problem in Eq.~\ref{eq:odiscriminator}\}}
		\STATE{Randomly initialise $\params_{0}$}
		\FOR{$i \in \langle 1, \ldots, \tau_{d} \rangle$}
		\STATE{$\emb{e} \leftarrow \emb{e} / \norm{\emb{e}}, \; \forall e \in \ents$}
		\STATE{$\batch \leftarrow \textsc{SampleBatch}(\KG, n)$}
		
		\STATE{$g_{i} \leftarrow  \nabla_{\params} \sum_{ \langle t, \tilde{t} \rangle \in \batch} \hinge{\gamma - \fscore(t ; \params_{i - 1}) + \fscore(\tilde{t} ; \params_{i - 1})}$}
		\STATE{$\qquad \quad + \; \lambda \loss_{G}(\bar{\mathbf{E}} ; \params)$}
		\STATE{$\params_{i} \leftarrow \params_{i - 1} - \eta_{i} g_{i}$}
		\ENDFOR
		\STATE{\textbf{return} $\params_{\tau}$}
	\end{algorithmic}
\end{algorithm}
%

%
The problem mentioned above can be avoided if, instead of enumerating $\BigO{\card{\ents}^{n}}$ entity tuples, we iteratively find a set of \emph{adversarial counter-examples} maximizing the loss function in Eq.~\ref{eq:lrule}, and then tune the model parameters $\params$ to minimize a linear combination of the losses in Eq.~\ref{eq:loss} and Eq.~\ref{eq:lrule}.
%


%
However, finding a tuple of entities $\langle e_{1}, \ldots, e_{n} \rangle \in \ents^{n}$ maximizing the loss in Eq.~\ref{eq:lrule} is a potentially intractable combinatorial problem.
%
Efficiently finding discrete adversarial examples is an open problem in adversarial training of neural architectures~\cite{1701.00160}.
%

%
In this work, we attack this problem by instead finding a tuple of \emph{adversarial entity embeddings} $\bar{\mathbf{E}} \triangleq \langle \aemb{1}, \ldots, \aemb{n} \rangle \in \Real^{k \times n}$ maximizing the loss in Eq.~\ref{eq:lrule} using gradient-based optimization methods~\cite{Goodfellow-et-al-2016}.
%
We will refer to the loss $\loss_{G}$ evaluated on the adversarial embeddings as $\loss_{G}(\bar{\mathbf{E}} ; \params)$.
%
For the sake of clarity, in the following we denote the score of a $\spo$ triple $\fscore(\spo ; \params)$ as $\fscore(\remb{\rp}, \emb{\rs}, \emb{\ro})$.
%

%
The resulting learning procedure, which we refer to as \emph{Adversarial Rule Injection} (\ARI), can be described as a minimax game where:
%
\begin{inparaenum}[1)]
% 
 \item One agent (the \emph{adversary}) finds a set of adversarial counter-examples maximizing the loss $\loss_{G}$ in Eq.~\ref{eq:lsimple}, and
%
 \item another agent (the \emph{discriminator}) tunes the model parameters $\params$ so to simultaneously minimize the losses $\loss$ in Eq.~\ref{eq:loss} and $\loss_{G}$ in Eq.~\ref{eq:lsimple}.
%
\end{inparaenum}
%

%
The training procedure in \ARI alternates between the following two objectives:
%
\begin{description}
%
 \item[Adversary:]
 %
 \begin{equation} \label{eq:oadversary}
 %
 \begin{aligned}
 & \underset{\Aemb}{\text{maximize}}
 & & \aloss(\Aemb) \triangleq \loss_{G}(\bar{\mathbf{E}} ; \params) \\
 & \text{subject to}
 & & \displaystyle{\forall \emb{} \in \Aemb \; \norm{\emb{}} = 1,}
 \end{aligned}
 %
 \end{equation}
 %
%
 \item[Discriminator:]
 %
 \begin{equation} \label{eq:odiscriminator}
 %
 \begin{aligned}
 & \underset{\params}{\text{minimize}}
 & & \dloss(\params) \triangleq \loss(\params) + \lambda \loss_{G}(\bar{\mathbf{E}} ; \params)\\
 & \text{subject to}
 & & \displaystyle{\forall e \in \ents: \; \norm{\emb{e}} = 1,}
 \end{aligned}
 %
 \end{equation}
 %
 %
%
\end{description}
%
\noindent where $\lambda \geq 0$ is a user-specified hyper-parameter specifying the weight of the rule-based loss in the training process.
%
The learning procedure in \ARI can thus be formalized by the following minimax problem:
%
\begin{equation} \label{eq:minimax}
%
 \min_{\params} \max_{\Aemb} \dloss(\params) + \aloss(\Aemb).
%
\end{equation}
%
In Alg.~\ref{alg:sgd} we provide an algorithm for solving the minimax problem in Eq.~\ref{eq:minimax}.
%

==> introduction.tex <==
% !TeX spellcheck = en_GB

\section{Introduction} \label{sec:introduction}

%
Knowledge Graphs are graph-structured Knowledge Bases, where facts are represented in the form of relationships between entities: they are powerful instruments in search, analytics and data integration.
%
Developments in the area of Knowledge Graphs were initially driven by academic efforts, such as \kg{DBpedia}~\cite{DBLP:conf/semweb/AuerBKLCI07}, \kg{Freebase}~\cite{DBLP:conf/aaai/BollackerCT07}, \kg{YAGO}~\cite{DBLP:conf/www/SuchanekKW07} and \kg{NELL}~\cite{DBLP:conf/aaai/CarlsonBKSHM10}.
%
At the time of this writing, Knowledge Graphs are also widely popular in industry applications, such as the \kg{Freebase}-based Google's Knowledge Graph\footnote{\url{https://developers.google.com/knowledge-graph/}} and Knowledge Vault~\cite{DBLP:conf/kdd/0001GHHLMSSZ14} projects, which support the company's search and smart assistance services.
%

%
However, despite the engineering efforts, real world Knowledge Graphs are often far from being complete.
%
For instance, consider \kg{Freebase}: 71\% of the persons described in the knowledge base have no known place of birth, 75\% have no known nationality, and coverage for less frequent relations can be even lower~\cite{DBLP:conf/kdd/0001GHHLMSSZ14}.
%
Similarly, in \kg{DBpedia} 66\% of the persons have no known place of birth, while 58\% of the scientists are missing a fact stating what they are known for~\cite{DBLP:conf/semweb/KrompassBT15}.
%

%
The problem of predicting missing links in knowledge graphs is known in the literature as \emph{link prediction} or \emph{Knowledge Base completion}. Many  successful link prediction methods operate on a local per-link basis: they assign a score to each possible candidate link. The score is calculated by feeding either learned or pre-trained entity and relation representations into neural architectures of different complexities~\cite{DBLP:conf/www/NickelTK12,DBLP:conf/nips/BordesUGWY13,DBLP:conf/naacl/RiedelYMM13,yang15:embedding,DBLP:conf/icml/TrouillonWRGB16}. 
This per-link approach has not just produced high accuracies on many benchmark datasets; it is also extremely efficient: After training, the cost of predicting a link is independent of graph size or connectivity. This can be contrasted with link prediction approaches that rely on graphical models and often require complex inference at test time.    

The simplicity of local models comes at a price: It is not obvious how to inject prior knowledge about graph properties that span more than one edge, such as transitivity, antisymmetry or more problem-specific rules. This is particularly unfortunate in scenarios were the training set is small and the model cannot learn such regularities from data. There is recent work that began to address this problem. Most of the relevant approaches~\cite{DBLP:conf/cikm/WangMC14,DBLP:conf/ijcai/WangWG15,DBLP:journals/corr/VendrovKFU15,DBLP:conf/akbc/RocktaschelR16} capture regularities using first-order rules such as \begin{equation*}
 \begin{aligned}
  \forall x, y, z: \rel{brotherOf}(x, y) \; \land \; \rel{parentOf}(y, z) \\ \implies \rel{uncleOf}(x, z).
 \end{aligned}
\end{equation*} 

These rules are then instantiated for all groundings of their free variables and turned into loss functions that measure grounded rule violations. Unfortunately, for large domains with many entities, this approach does not scale. For example, the above rule  unrolls into a billion groundings for a thousand entities. One can sub-sample, but in practice most groundings are trivially satisfied, and hence their loss gradients disappear. This makes learning slow. Some work has managed to avoid grounding~\cite{DBLP:conf/emnlp/DemeesterRR16}, but only for a very limited set of models and rules. For example, the family relationship rule above would not be supported.  

In this paper we show that link predictors can be regularised to capture prior knowledge in a way that is both \emph{general} and \emph{scalable}. The underlying idea is the following: Instead of forcing the model to minimise a loss on all groundings, it should only minimise the loss of a \emph{worst offender}. Moreover, instead of a combinatorial search over Cartesian products of all entities, we solve a (non-convex) continuous optimisation problem over the infinite space of entity \emph{representations}. While this generally cannot be solved to optimality, we have effective and generic methods to reliably find local optima. A side effect of this approach is that the representations of actual entities never appear in the constraint-specific loss terms. Hence, the model cannot easily overfit by changing specific entity representations to fulfil constraints. 

We capture the above ideas in an adversarial training regime with two players. The first player is the link predictor. The predictor is given a collection of actual training entities and needs to predict a set of edges that match the training graph. The predictor also receives a set of \emph{synthetic} entity representations. On these synthetic representations the predictor needs to predict a graph that is consistent with the given prior assumptions. The second player is an adversarial to the first: it needs to produce \emph{synthetic} entity representations on which the predictor fails to construct a consistent graph. The game is played by optimising a mix-max objective, akin to GAN training.    

We evaluate our approach on several datasets, types of prior constraints and models. We observe that our approach indeed scales better than previous generic methods, leading to higher accuracies faster. \ttodo{}

The paper is organised as follows. We will first give a brief introduction to the link prediction and the models we consider. Then we introduce our adversarial method, compare it to related work, and evaluate it empirically on a range of datasets. 

% In \cite{DBLP:conf/naacl/RocktaschelSR15}, the authors regularize entity-tuple and relation embeddings via First-Order Logic rules: every rule is propositionalized, and a differentiable loss term is added for every propositional rule.
% %
% However, this approach does not scale to large knowledge bases: even a simple rule such as
% %
% \begin{equation*}
%  \begin{aligned}
%   \forall x, y, z: \rel{brotherOf}(x, y) \; \land \; \rel{parentOf}(y, z) \\ \implies \rel{uncleOf}(x, z)
%  \end{aligned}
% \end{equation*}
% %
% \noindent would result in a very large number of loss terms.
% %
% In \cite{DBLP:conf/emnlp/DemeesterRR16} this problem is overcome by minimizing an upper bound of the loss that encourages the implication between relations to hold, entirely independent from the number of entities.
% %
% However, their approach -- a variant of \mdl{Model F}~\cite{DBLP:conf/naacl/RiedelYMM13} -- is only able to model a very restricted set of rules in the form:
% %
% \[ \forall x, y : \rp(x, y) \implies \relq(x, y), \]
% %
% \noindent where $\rp$ and $\relq$ are two arbitrary relations.
% %  


% rely on learned distributed vector representations of entities and relations in the Knowledge Graph~\cite{DBLP:conf/www/NickelTK12,DBLP:conf/nips/BordesUGWY13,DBLP:conf/naacl/RiedelYMM13,yang15:embedding,DBLP:conf/icml/TrouillonWRGB16}.




% Therefore, in this paper we focus on the problem of \emph{predicting missing links} in Knowledge Graphs, so to discover new facts: in the literature, this problem is also known as \emph{link prediction} and \emph{Knowledge Base completion}.
% %
% Current successful link prediction methods heavily rely on learned distributed vector representations of entities and relations in the Knowledge Graph~\cite{DBLP:conf/www/NickelTK12,DBLP:conf/nips/BordesUGWY13,DBLP:conf/naacl/RiedelYMM13,yang15:embedding,DBLP:conf/icml/TrouillonWRGB16}.
% %
% We refer to \cite{DBLP:journals/pieee/Nickel0TG16} for a detailed description of such methods.
% %
% Although such models are able to learn robust representations of entities and relations from large amount of data, they lack common-sense knowledge and reasoning.
% %

% \subsection{Related Works}

% %
% Combining neural methods with symbolic common-sense knowledge, \eg in the form of implication rules, is an actively researched area~\cite{DBLP:conf/cikm/WangMC14,DBLP:conf/ijcai/WangWG15,DBLP:journals/corr/VendrovKFU15,DBLP:conf/akbc/RocktaschelR16,DBLP:conf/emnlp/DemeesterRR16}.
% %
% In \cite{DBLP:conf/naacl/RocktaschelSR15}, the authors regularize entity-tuple and relation embeddings via First-Order Logic rules: every rule is propositionalized, and a differentiable loss term is added for every propositional rule.
% %
% However, this approach does not scale to large knowledge bases: even a simple rule such as
% %
% \begin{equation*}
%  \begin{aligned}
%   \forall x, y, z: \rel{brotherOf}(x, y) \; \land \; \rel{parentOf}(y, z) \\ \implies \rel{uncleOf}(x, z)
%  \end{aligned}
% \end{equation*}
% %
% \noindent would result in a very large number of loss terms.
% %
% In \cite{DBLP:conf/emnlp/DemeesterRR16} this problem is overcome by minimizing an upper bound of the loss that encourages the implication between relations to hold, entirely independent from the number of entities.
% %
% However, their approach -- a variant of \mdl{Model F}~\cite{DBLP:conf/naacl/RiedelYMM13} -- is only able to model a very restricted set of rules in the form:
% %
% \[ \forall x, y : \rp(x, y) \implies \relq(x, y), \]
% %
% \noindent where $\rp$ and $\relq$ are two arbitrary relations.
% %

% \subsection{Contribution}

% %
% \emph{Adversarial examples} are examples crafted for significantly increasing the loss functional of a machine learning model, while \emph{adversarial training} is the process of training a model to correctly classify both training and adversarial examples~\cite{szegedy14:intriguing,goodfellow15:harnessing}.
% %

% %
% In this paper we present a method, named \emph{Adversarial Rule Injection} (\ARI), for incorporating general First-Order Logic rules in Knowledge Graph embedding models.
% %
% \ARI relies on an \emph{adversarial training architecture}, where:
% %
% \begin{inparaenum}[1)]
% %
%  \item An \emph{adversary} finds counter-examples that maximize a rule violation loss, and
% %
%  \item a \emph{discriminator} tunes the parameters such as to minimize the rule violation loss on these counter-examples.
% %
% \end{inparaenum}
% %

% %
% In particular, in \ARI, counter-examples are found in the \emph{continuous embedding space} rather than in the discrete fact space.
% %
% This has several advantages, namely:
% %
% \begin{description}
% %
%  \item[Scalability:] It decouples the complexity of the method from the number of entities in the Knowledge Base, which can be in the order of millions or more.
% %
%  \item[Generalizability:] It enforces rules to hold everywhere in the embedding space, even on previously unseen entity embeddings.
% %
%  \item[Flexibility:] It can be used jointly with any Knowledge Graph embedding model, without making any assumption on its architecture.
% %
% \end{description}
% %

% %
% In Statistical Relational Learning~\cite{getoor:srlbook07}, the proposed approach falls in the category of \emph{lifted inference and learning}~\cite{DBLP:conf/ijcai/Poole03,DBLP:conf/ijcai/BrazAR05}: by imposing the desired constraints on the whole entity embedding space, we can efficiently reason about groups of objects as a whole by exploiting symmetries in the relational structure of the model.
% %
% This allows imposing a large number of First-Order rules while learning the distributed representations of all entities and relations in the Knowledge Graph.
% %
% Two fundamental advantages with respect to the method in \cite{DBLP:conf/naacl/RocktaschelSR15} are the drastically lower computation times and the fact that rules are enforced to hold on the whole embedding space, even on previously unseen entity embeddings -- thus covering the cases where not all entity embeddings are visible at training time, such as in Row-Less Universal Schema~\cite{DBLP:journals/corr/VergaM16}.
% %
% The method in \cite{DBLP:conf/emnlp/DemeesterRR16} is also \emph{lifted}, but can only handle a very small subset of First-Order rules.
% %

